Characterizing Continuous Time Random Walks on Time Varying Graphs

In this paper we study the behavior of a continuous time random walk (CTRW) on a stationary and ergodic time varying dynamic graph. We establish conditions under which the CTRW is a stationary and ergodic process. In general, the stationary distribution of the walker depends on the walker rate and is difficult to characterize. However, we characterize the stationary distribution in the following cases: i) the walker rate is significantly larger or smaller than the rate in which the graph changes (time-scale separation), ii) the walker rate is proportional to the degree of the node that it resides on (coupled dynamics), and iii) the degrees of node belonging to the same connected component are identical (structural constraints). We provide examples that illustrate our theoretical findings.

==> figs/static_SlowCTRWa.tex <==
\vspace{-10pt}
\begin{tikzpicture}[scale=1.4,every node/.style={minimum size=4.5mm,circle,fill=blue!20}]

\domath{0}{\offset}

\dointmath{4}{\N}
\dointmath{\N-1}{\ang}

\node  (1) at (\offset+0,0) {};
\node  (mn1) [fill=none] at (\offset+0,0) {$\frac{1}{2}$};

\foreach \n in {2,...,\N}{%
\domath{\offset+1*sin(\n*360/\ang)}{\x}
\domath{1*cos(\n*360/\ang)}{\y}
\node (\n) at (\x,\y) {};
\node (mn\n) [fill=none] at (\x,\y) {$\frac{1}{6}$};
};

\path[->] (1) edge [out=35, in=10,loop] node [above, fill=none] {$\frac{2}{3}$} (1);

\path[->] (2) edge [out=165, in=135,loop] node [above, fill=none] {$\frac{2}{3}$} (2);


\path[->] (1) edge [bend left] node [right, fill=none] {$\frac{1}{9}$} (2);
\path[->] (2) edge [bend left] node [left, fill=none] {$\frac{1}{3}$} (1);

\foreach \n in {3,...,\N} {
\path[dotted,->] (\n) edge [out=45, in=65,loop] (\n);
\path[dotted,->] (1) edge [bend left] (\n);
\path[dotted,->] (\n) edge [bend left] (1);
};

\end{tikzpicture}


==> figs/static_SlowCTRWb.tex <==
\vspace{-10pt}
\begin{tikzpicture}[scale=1.4,auto=left,every node/.style={minimum size=4.5mm,circle,fill=blue!20}]

\domath{0}{\offset}

\dointmath{4}{\N}
\dointmath{\N-1}{\ang}

\node  (1) at (\offset+0,0) {};
\node  (mn1) [fill=none] at (\offset+0,0) {$\frac{1}{4}$};

\foreach \n in {2,...,\N}{%
\domath{\offset+1*sin(\n*360/\ang)}{\x}
\domath{1*cos(\n*360/\ang)}{\y}
\node (\n) at (\x,\y) {};
\node (mn\n) [fill=none] at (\x,\y) {$\frac{1}{4}$};
};

\path[->] (2) edge [out=165, in=135,loop] node [above, fill=none] {$\frac{2}{3}$} (2);

\path[->] (1) edge [bend left] node [right, fill=none] {$\frac{1}{3}$} (2);
\path[->] (2) edge [bend left] node [left, fill=none] {$\frac{1}{3}$} (1);

\foreach \n in {3,...,\N} {
\path[dotted,->] (\n) edge [out=45, in=65,loop] (\n);
\path[dotted,->] (1) edge [bend left] (\n);
\path[dotted,->] (\n) edge [bend left] (1);
};

\end{tikzpicture}


==> figs/static_Weighted.tex <==
\begin{tikzpicture}[scale=1.2,every node/.style={minimum size=4.5mm,circle,fill=blue!20}]

\domath{0}{\offset}
\dointmath{4}{\N}
\dointmath{\N-1}{\ang}

\node  (1) at (\offset+0,0) {};
\node  (mn1) [fill=none] at (\offset+0,0) {$\frac{1}{2}$};

\foreach \n in {2,...,\N}{%
\domath{\offset+1*sin(\n*360/\ang)}{\x}
\domath{1*cos(\n*360/\ang)}{\y}
\node (\n) at (\x,\y) {};
\node (mn\n) [fill=none] at (\x,\y) {$\frac{1}{6}$};
};

\foreach \n in {2,...,\N}
\path[draw,-] (1) -- node[font=\tiny,shape=rectangle,fill=white] {$\frac{1}{\ang}$} (\n);

\end{tikzpicture}


==> figs/static_dyn_example1.tex <==
\begin{tikzpicture}[scale=.8,auto=left,every node/.style={minimum size=4.5mm,circle,fill=blue!20}]

\newcommand{\circlesize}{2.2cm}
\domath{1.6}{\writing}

\node [fill=none,draw,circle,minimum size=\circlesize] (s1) at (0,0) {};

\domath{0}{\offset}

\dointmath{4}{\N}
\dointmath{\N-1}{\ang}

\node  (1) at (\offset+0,0) {};
\node  (mn1) [fill=none] at (\offset+0,0) {$\frac{1}{6}$};

\foreach \n in {2,...,\N}{%
\domath{\offset+1*sin(\n*360/\ang)}{\x}
\domath{1*cos(\n*360/\ang)}{\y}
\node (\n) at (\x,\y) {};
\node (mn\n) [fill=none] at (\x,\y) {$\frac{1}{18}$};
};

\foreach \n in {2,...,\N}
\draw[thick,color=red] (1) -- (\n);

%\node [fill=none] (t1) at (\offset,-\writing) {\small $E[S_1] = 1$};
\node [fill=none] (n1) at (\offset,\writing) {$G_1$};


\domath{3.5}{\offset}

\node [fill=none,draw,circle,minimum size=\circlesize] (s2) at (\offset,0) {};

\dointmath{\N+1}{\Nb}
\dointmath{2*\N}{\Ne}

\node  (\Nb) at (\offset+0,0) {};
\node  (mn\Nb) [fill=none] at (\offset+0,0) {$\frac{1}{6}$};


\domath{\Nb+1}{\Nbp}

\foreach \n in {\Nbp,...,\Ne}{%
\domath{\offset+1*sin(\n*360/\ang)}{\x}
\domath{1*cos(\n*360/\ang)}{\y}
\node (\n) at (\x,\y) {};
\node (mn\n) [fill=none] at (\x,\y) {$\frac{1}{18}$};
};

%\node [fill=none] (t2) at (\offset,-\writing) {\small $E[S_2] = 1$};
\node [fill=none] (n2) at (\offset,\writing) {$G_2$};


\path[->] (s1) edge [bend left] (s2);
\path[->] (s2) edge [bend left] (s1);



\domath{\offset + 1.75}{\offset}

% \node [fill=none] (sn) at (\offset,0) {$\dots$};

\domath{\offset + 1.75}{\offset}

\node [fill=none,draw,circle,minimum size=\circlesize] (s3) at (\offset,0) {};

\dointmath{\Ne+1}{\Neb}
\dointmath{\Ne+\N}{\Nee}

\node  (\Neb) at (\offset+0,0) {};
\node  (mn\Neb) [fill=none] at (\offset+0,0) {$\frac{1}{6}$};

\dointmath{\Neb+1}{\Nebp}

\foreach \n in {\Nebp,...,\Nee}{%
\domath{\offset+1*sin(\n*360/\ang)}{\x}
\domath{1*cos(\n*360/\ang)}{\y}
\node (\n) at (\x,\y) {};
\node (mn\n) [fill=none] at (\x,\y) {$\frac{1}{18}$};
};

%\node [fill=none] (t3) at (\offset,-\writing) {\small $E[S_\ang] = 1$};
\node [fill=none] (n3) at (\offset,\writing) {$G_\ang$};

\path[->] (s1) edge [bend left] (s3);
\path[->] (s2) edge [bend left] (s3);

\path[->] (s3) edge [bend left] (s1);
\path[->] (s3) edge [bend left] (s2);

\end{tikzpicture}


==> figs/static_dyn_example2.tex <==
\begin{tikzpicture}[scale=.8,auto=left,every node/.style={minimum size=4.5mm,circle,fill=blue!20}]

\newcommand{\circlesize}{2.2cm}
\domath{1.6}{\writing}

\node [fill=none,draw,circle,minimum size=\circlesize] (s1) at (0,0) {};

\domath{0}{\offset}

\dointmath{4}{\N}
\dointmath{\N-1}{\ang}

\node  (1) at (\offset+0,0) {};
\node  (mn1) [fill=none] at (\offset+0,0) {$\frac{1}{12}$};

\foreach \n in {2,...,\N}{%
\domath{\offset+1*sin(\n*360/\ang)}{\x}
\domath{1*cos(\n*360/\ang)}{\y}
\node (\n) at (\x,\y) {};
\node (mn\n) [fill=none] at (\x,\y) {$\frac{1}{12}$};
};

\draw[thick,color=red] (1) -- (\N);

%\node [fill=none] (t2) at (\offset,-\writing) {\small $E[S_1] = 1$};
\node [fill=none] (n2) at (\offset,\writing) {$G_1$};

\domath{3.5}{\offset}

\node [fill=none,draw,circle,minimum size=\circlesize] (s2) at (\offset,0) {};

\dointmath{\N+1}{\Nb}
\dointmath{2*\N}{\Ne}

\node  (\Nb) at (\offset+0,0) {};
\node  (mn\Nb) [fill=none] at (\offset+0,0) {$\frac{1}{12}$};

\dointmath{\Nb+1}{\Nbp}

\foreach \n in {\Nbp,...,\Ne}{%
\domath{\offset+1*sin(\n*360/\ang)}{\x}
\domath{1*cos(\n*360/\ang)}{\y}
\node (\n) at (\x,\y) {};
\node (mn\n) [fill=none] at (\x,\y) {$\frac{1}{12}$};
};

\draw[thick,color=red] (\Nb) -- (\Ne);

%\node [fill=none] (t2) at (\offset,-\writing) {\small $E[S_2] = 1$};
\node [fill=none] (n2) at (\offset,\writing) {$G_2$};


\path[->] (s1) edge [bend left] (s2);
\path[->] (s2) edge [bend left] (s1);



\domath{\offset + 1.75}{\offset}

% \node [fill=none] (sn) at (\offset,0) {$\dots$};

\domath{\offset + 1.75}{\offset}

\node [fill=none,draw,circle,minimum size=\circlesize] (s3) at (\offset,0) {};

\dointmath{\Ne+1}{\Neb}
\dointmath{\Ne+\N}{\Nee}

\node  (\Neb) at (\offset+0,0) {};
\node  (mn\Neb) [fill=none] at (\offset+0,0) {$\frac{1}{12}$};

\dointmath{\Neb+1}{\Nebp}

\foreach \n in {\Nebp,...,\Nee}{%
\domath{\offset+1*sin(\n*360/\ang)}{\x}
\domath{1*cos(\n*360/\ang)}{\y}
\node (\n) at (\x,\y) {};
\node (mn\n) [fill=none] at (\x,\y) {$\frac{1}{12}$};
};

\draw[thick,color=red] (\Neb) -- (\Nee);

%\node [fill=none] (t3) at (\offset,-\writing) {\small $E[S_\ang] = 1$};
\node [fill=none] (n3) at (\offset,\writing) {$G_\ang$};

\path[->] (s1) edge [bend left] (s3);
\path[->] (s2) edge [bend left] (s3);

\path[->] (s3) edge [bend left] (s1);
\path[->] (s3) edge [bend left] (s2);

\end{tikzpicture}

